DeAR: Dual-Stage Document Reranking with Reasoning Agents via LLM Distillation

Large Language Models (LLMs) have transformed listwise document reranking by enabling global reasoning over candidate sets, yet single models often struggle to balance fine-grained relevance scoring with holistic cross-document analysis. We propose \textbf{De}ep\textbf{A}gent\textbf{R}ank (\textbf{\DeAR}), an open-source framework that decouples these tasks through a dual-stage approach, achieving superior accuracy and interpretability. In \emph{Stage 1}, we distill token-level relevance signals from a frozen 13B LLaMA teacher into a compact \{3, 8\}B student model using a hybrid of cross-entropy, RankNet, and KL divergence losses, ensuring robust pointwise scoring. In \emph{Stage 2}, we attach a second LoRA adapter and fine-tune on 20K GPT-4o-generated chain-of-thought permutations, enabling listwise reasoning with natural-language justifications. Evaluated on TREC-DL19/20, eight BEIR datasets, and NovelEval-2306, \DeAR surpasses open-source baselines by +5.1 nDCG@5 on DL20 and achieves 90.97 nDCG@10 on NovelEval, outperforming GPT-4 by +3.09. Without fine-tuning on Wikipedia, DeAR also excels in open-domain QA, achieving 54.29 Top-1 accuracy on Natural Questions, surpassing baselines like MonoT5, UPR, and RankGPT. Ablations confirm that dual-loss distillation ensures stable calibration, making \DeAR a highly effective and interpretable solution for modern reranking systems.\footnote{Dataset and code available at https://github.com/DataScienceUIBK/DeAR-Reranking.}.

==> tables/listwise_table.tex <==


\begin{table*}[!t]
\centering
\scriptsize
\setlength\tabcolsep{0.5pt}

\begin{tabular}{l| cc | cccccccc | c }

\toprule
\textbf{Method} & DL19 & DL20 & Covid &  NFCorpus &  Touche &  DBPedia & SciFact &  Signal & News &  Robust04 & BEIR (Avg) \\

\midrule




RankGPT (gpt-4)
& 75.59 & 70.56 & 85.51 & 38.47 & 38.57 & 47.12 & 74.95 & 34.40 & 52.89 & 57.55 & 53.68
\\



% \midrule
% \multicolumn{5}{l}{2st stage Reranking (Listwise) LLAMA 3.1 8b}\\
% \midrule

% \code{DistillRank\_$T_{13B}S_{8B}$\_RL}
% & 73.96  & 71.63 & 87.11  & 39.41 & 32.58 &  46.53  &  77.74 & 32.81 & 54.69 & 59.31 & 53.77
% %metrices_llama3.1_final_30_length_30000_documents

% \\  
% \code{DistillRank\_$T_{13B}S_{8B}$\_BC}
% & 74.55  & 69.82  & 87.11  & 38.58 &  33.37 &  46.51  & 78.82 & 32.22  & 53.07 & 59.66 & 53.66
% %metrices_llama3.1_final_30000_documents.json
% \\  
% \code{DistillRank\_$T_{13B}S_{3B}$\_RL}

% %metrices_Llama-3.1_32_64_0.1_50000
% & 75.85 & 71.35 & 87.89 & 38.61 & 33.29 & 46.98 & 77.40 & 32.60 & 54.38 & 57.88 & 53.64


% \\  
% %\code{DistillRank\_$T_{13B}S_{3B}$\_BC}
% %& 74.89  &  70.48 & 87.23  & 38.49 &  34.31 &  46.17 &77.18  & 31.78 & 51.69  &  58.84 &  53.21
% \code{DistillRank\_$T_{13B}S_{3B}$\_BC}
% %metrices_llama3.1_final_30000_documents
% & 74.89 & 70.48 & 87.24 & 38.50 & 34.31 & 46.17 & 77.18 & 31.78 & 51.70 & 58.84 & 53.29
% \\  
\midrule
\multicolumn{12}{c}{DeepAgentRank-Listwise (CoT GPT)}\\
\midrule

\code{P-Llama3.1-8B-RL \rightarrow  GPT-4} & 75.74 & 72.18 & 86.28 & \textbf{40.56} & 31.41 & 46.15 & 77.58 & 31.13 & 50.77 & 57.91 & 53.44 \\
\code{P-Llama3.1-8B-BC \rightarrow  GPT-4} & 75.68 & \textbf{72.73} & 86.12 & 40.42 & 31.60 & 45.99 & 78.36 & 32.40 & 52.10 & \textbf{62.18} & 53.65 \\
\code{P-Llama3.2-3B-RL \rightarrow  GPT-4}  & 74.72 & 72.21 & 85.13 & 40.30 & 33.95 & 46.17 & 78.04 & 31.79 & 53.28 & 60.25 & 53.64 \\
\code{P-Llama3.2-3B-BC \rightarrow  GPT-4} & \textbf{76.29} & 70.88 & 85.79 & 40.34 & 32.43 & 45.79 & 76.71 & 33.00 & 52.76 & 60.39 & 53.48 \\

% \midrule
% \multicolumn{5}{l}{2st stage Reranking (Listwise) COT GPT}\\
% \midrule


%\code{DistillRank\_$T_{13B}S_{8B}$\_BC}
%&  75.67 & 70.98 & 87.19 & 40.58 & 32.50 & 46.45 & 77.25 & 33.51 & 50.63 & 61.04 & 53.67
%llama8_passage2/rankllama_teacher_13b_student_8b_msmacroo_0.1_2/checkpoint-1000


\midrule
\multicolumn{12}{c}{DeepAgentRank-Listwise (CoT Llama3.1 8B)}\\
\midrule

\code{P-Llama3.1-8B-RL \rightarrow  Llama3.1 8B} & 74.86 & 71.06 & 86.43 & 39.08 & 33.76 & 46.61 & 78.08 & 33.10 & 53.17 & 59.55 & 53.77 

%metrices_Llama-3.1-8B-Instruct-lora-8-cot-checkpoint-7000_part1
%metrices_Llama-3.1-8B-Instruct-lora-8-cot-checkpoint-7000_part2
\\  
\code{P-Llama3.1-8B-BC \rightarrow  Llama3.1 8B}  & 75.54 & 70.39 & 86.53 & 38.48 & 34.32 & 46.20 & \textbf{78.47} & 31.69 & \textbf{53.79} & 59.43 & 53.67 
%metrices_Llama-3.1-8B-Instruct-lora-8-cot-checkpoint-7000
\\  
\code{P-Llama3.1-3B-RL \rightarrow  Llama3.1 8B} & 75.29 & 71.17 & 88.10 & 39.05 & 31.47 & 46.69 & 77.77 & 32.64 & 53.09 & 57.93 & 53.35 
%metrices_Llama-3.1_32_64_0.1_50000_cot

\\  

%metrices_Llama-3.1_32_64_0.1_50000_cot
\code{P-Llama3.1-3B-BC \rightarrow  Llama3.1 8B} & 75.33 & 70.02 & \textbf{88.36} & 38.80 & \textbf{35.04} & 46.34 & 77.34 & \textbf{32.56} & 52.24 & 58.63 & 53.61 
%metrices_Llama-3.1_32_64_0.1_50000_cot
\\ 
\bottomrule
\end{tabular}


\caption{Listwise reranking performance (nDCG@10) on TREC Deep Learning Tracks 2019 (DL19), 2020 (DL20), and BEIR datasets (CovidQA, NFCorpus, Touche, DBPedia, SciFact, Signal, News, Robust04). DeepAgentRank-Listwise re-ranks the top-30 passages from the pointwise stage, using CoT reasoning from GPT-4o (CoT GPT) or Llama-3.1 (CoT Llama). Labels indicate the pointwise model (e.g., Llama 8B RankLoss) and listwise configuration (e.g., Llama-3.1 8B RL). Best scores per dataset are bolded.}
\label{table:list-wise-benchmark
}
\label{table:list-wise-benchmark}

\end{table*}

==> tables/pointwise_table.tex <==


\begin{table*}[!t]
\centering
\scriptsize
\setlength\tabcolsep{0.5pt}

\begin{tabular}{l| cc | cccccccc | c }

\toprule
\textbf{Method} & DL19 & DL20 & Covid &  NFCorpus &  Touche &  DBPedia & SciFact &  Signal & News &  Robust04 & BEIR (Avg) \\

\midrule

BM25
& 50.58 & 47.96 & 59.47 & 30.75 & \textbf{44.22} & 31.80 & 67.89 & 33.05 & 39.52 & 40.70 & 43.42
\\

\midrule

\multicolumn{12}{c}{\textbf{Supervised}}\\ 

\midrule

monoBERT (340M)
& 70.50 & 67.28 & 70.01 & 36.88 & 31.75 & 41.87 & 71.36 & 31.44 & 44.62 & 49.35 & 47.16
\\

monoT5 (220M)
& 71.48 & 66.99 & 78.34 & 37.38 & 30.82 & 42.42 & 73.40 & 31.67 & 46.83 & 51.72 & 49.07
\\

monoT5 (3B)
& 71.83 & 68.89 & 80.71 & \textbf{38.97} & 32.41 & 44.45 &  \textbf{76.57} & 32.55 & 48.49 & 56.71 & 51.36
\\


Cohere Rerank-v2
& 73.22 & 67.08 & 81.81 & 36.36 & 32.51 & 42.51 & 74.44 & 29.60 & 47.59 & 50.78 & 49.45
\\

%TART-Rerank (3B)
% &67.43 & 59.19 & 72.80 & 33.40 & 24.90 & 46.80 & 77.70 & - &- & -&-
% \\
%RankT5 (3B)
%& -& -& 80.71 &38.10 &44.01 & 44.22&  74.99&  32.00& - & -&
% \\



 



\midrule
\multicolumn{12}{c}{\textbf{Unsupervised}}\\ 
\midrule

UPR (3B)
& 53.85 & 56.02 & 68.11 & 35.04 & 19.69 & 30.91 & 72.69 & 31.91 & 43.11 & 42.43 & 42.99
\\

% SGPT-CE (6.1B)
% & 79.1 & 34.7 & 23.4 & 37.0 & 68.2 & 32.3 & 46.6 & 48.0 & 46.16
% \\

InPars (3B)
& - & 66.12 &  78.35 & - & - & - & - & - & - & - & -
\\

% HyDE (\code{text-davinci-003})
% & 59.3 & - & 27.3 & - & 44.0 & - & 46.6 & - & 36.8 & 69.1
% \\

% Promptagator++ (zero-shot)$^\dagger$
% & - & - & 76.0 & 36.0 & 27.8 & 41.3 & 73.6 & - & - & - & -
% \\

Promptagator++
& - & - & 76.2 & 37.0 & 38.1 & 43.4 & 73.1 & - & - & - & -
\\


%\midrule
%\multicolumn{5}{l}{LLM API (Permutation generation)}\\
%\midrule

\code{RankGPT (gpt-3.5-turbo)}
& 65.80 & 62.91  & 76.67 & 35.62 & 36.18 & 44.47 & 70.43 & 32.12 & 48.85 & 50.62 & 49.37
\\

% \code{gpt-4}$^\dagger$
% & \textbf{75.59} & \textbf{70.56} & \textbf{85.51} & \textbf{38.47} & \textbf{38.57} & \textbf{47.12} & \textbf{74.95} & \textbf{34.40} & \textbf{52.89} & \textbf{57.55} & \textbf{53.68}
% \\

\midrule
\multicolumn{11}{c}{\textbf{ DeepAgentRank-Pointwise}} \\
\midrule
\code{P-Llama3.1-8B-RL} & 72.17 & 68.93 & 85.21 & 37.01 & 34.88 & 45.56 & 77.43 & 30.16 & 52.05 & 54.42 & 52.09 \\
\code{P-Llama3.1-8B-BC} & 74.50 & 68.71 & 84.14 & 36.57 & 37.23 & 46.27 & 77.39 & 29.91 & 51.71 & 52.43 & 51.95 \\
\code{P-Llama3.1-3B-RL} & 72.94 & 69.21 & 83.01 & 36.30 & 35.76 & 45.96 & 74.45 & 28.64 & 50.84 & 49.78 & 50.59 \\
\code{P-Llama3.1-3B-BC} & 74.49 & 69.02 & 82.91 & 35.78 & 36.17 & 45.28 & 75.48 & 29.14 & 48.99 & 50.93 & 50.58 \\




\bottomrule
\end{tabular}


\caption{Pointwise reranking performance (nDCG@10) on TREC Deep Learning Tracks 2019 (DL19), 2020 (DL20), and BEIR datasets (CovidQA, NFCorpus, Touche, DBPedia, SciFact, Signal, News, Robust04). DeepAgentRank-Pointwise uses a Llama-2 13B teacher with student models (Llama 8B or Llama-3.2 3B) trained with RankLoss (e.g., RankNet) or Binary Cross-Entropy (Binary CE). "-" indicates unavailable results. Best scores per dataset are bolded.}
\label{table:benchmark}
\end{table*}
